A novel set of rotationally and translationally invariant features for images based on the non-commutative bispectrum

We propose a new set of rotationally and translationally invariant features for image or pattern recognition and classification. The new features are cubic polynomials in the pixel intensities and provide a richer representation of the original image than most existing systems of invariants. Our construction is based on the generalization of the concept of bispectrum to the three-dimensional rotation group SO(3), and a projection of the image onto the sphere.

==> projection.tex <==
\section{A projection onto the sphere}

\ignore{
The natural invariance group of images is the Euclidean group \m{\mathrm{ISO}^{+}(2)} of rigid body motions in the plane. 
To make this statement more precise, %we start out with a continuous representation of images. 
given an \m{N\times N} pixel monochrome bitmap image \m{x}, %by some appropriate smoothing and rescaling procedure,  
we associate to \m{x} a continuous function \m{f\colon \RR^2\to \sqb{0,1}} such that for \m{1\<\leq i,j\<\leq N},~ 
\m{f(\fr{i-1/2}{N},\fr{j-1/2}{N})} is proportional to the intensity of pixel \m{(i,j)}, and
\m{f} drops off to zero outside of \m{\sqb{0,1}^2}. What exact interpolation procedure we use to construct \m{f} 
is at this stage immaterial, as long as \m{f} is reasonably smooth. 

Now \m{\ISOtwo}
}

\ignore{
Monochrome images are commonly represented either as \m{N\times N} arrays of pixel intensities or as 
continuous functions \m{h\colon \RR^2\to\sqb{0,1}} with support confined to a compact region, 
for example, the square \m{\sqb{-0.5,0.5}^2}. % \m{B=\sqb{0,1}^2}.  
For our purposes, the continuous representation is more natural.  
%For now, we leave open the exact form of interpolation used to arrive at it from the bitmap, 
% is largely immaterial. For now we 
%only 
We further assume that \m{h\in L_2(\RR^2)}. 

The natural invariance group for images is the Euclidean group \m{\mathrm{ISO}^{+}(2)} of rigid body motions in the plane. 
Each group element \m{T\in\ISOtwo} may be written as a rotation by some angle \m{\theta} 
followed by a translation by some vector \m{\br{b_1,b_2}^\top}:  
\begin{equation*}
    T\colon \Matrix{x\\y} \mapsto \Matrix{\cos \theta & - \sin\theta \\ \sin\theta & \cos\theta} \Matrix{x\\y}+
    \Matrix{b_1\\b_2}. 
\end{equation*}
%Applying such a transformation to \m{f}, we have we have \m{Tf(x)}
This induces an action on functions \m{h\mapsto h'=T(h)} \ignore{of \m{\ISOtwo}} with %by defining %\m{f'=T(f)} via the relation 
\m{h'(T(x))=h(x)}, i.e., \m{h'(x)=h(T^{-1}(x))}. We say that a kernel \m{k} between 
images is invariant to the Euclidean group if for any pair of images \m{h_1} and \m{h_2}, and any \m{T\in\ISOtwo}, 
\m{k(h_1,h_2)=k(h_1,T(h_2))=k(T(h_1),h_2)}. 
A learning algorithm based on such a kernel 
%is truly invariant to translation and rotation, in the sense that 
%has the perty that it 
will treat rotated and translated versions of an image as identical, 
regardless of the extent of rotation and translation, and regardless of the center of the rotation. 

Unfortunately, \m{\ISOtwo} itself is not amenable to the algebraic 
technique of constructing invariants presented in this paper, because it 
is not a compact group. This, in turn, is related to the fact that \m{\RR^2} is not a compact space, and suggests  
%This motivates 
 projecting  to a different space, namely %the space of functions on 
the unit sphere \m{S_2}. 
%The sphere is locally isomorphic to \m{\RR^2}, and its usual coordinate-system, the spherical polars 
%The sphere is commonly parametrized by spherical polar coordinates \m{(\theta,\phi)},~ \m{\0\<\leq \theta < < \pi} and 
%\m{0\<\leq \phi\< < 2\pi}. 
%Since \m{S_2} is locally isomorphic to \m{\RR^2} and 

The support of \m{h} being restricted to \m{\sqb{-0.5,0.5}^2}, 
a simple and relatively low distortion mapping \m{L_2(\RR^2)\to L_2(S_2)} %,~\m{f\mapsto \tilde f} 
%this can be done easily and 
%with relatively little distortion 
is not difficult to construct. %, for example, % by setting %the map
%To define our mapping, 
We take 
\begin{equation}\label{eq: mapping}
  h\mapsto f, \qquad 
  f(\theta,\phi)=h(r_{\RR^2},\theta_{\RR^2})=h(\tovr{a} \theta,\phi),  
\end{equation}
where \m{ 0\<\leq \theta \< \leq \pi} and \m{0\<\leq \phi\< < 2\pi} are spherical polar coordinates, 
while \m{r_{\RR^2}\<=\ovr{a}\theta} and \m{\theta_{\RR^2}\<=\phi} are planar polars, and \m{a} 
is a numerical parameter, typically around 0.3 (Figure \ref{fig: projection}). 
\begin{figure}[htbp]
  \centering
  
  \caption{The projection of an image onto the sphere \m{S_2}. 
    Rotations of the sphere correspond to translations and rotations of the original image.}
  \label{fig: projection}
\end{figure}
The smaller \m{a} is, the less distortion we suffer, but %as it will become clear in the next section,  
the more numerical work we have to perform to achieve the same resolution. 

To numerically represent \m{f}, we use \df{spherical harmonics} 
\begin{equation*}
  Y_l^m(\theta,\phi)= \sqrt{\fr{2l+1}{4\pi}\fr{\br{l-m}!}{\br{l+m}!}}~~ P_l^m(\cos \theta)~ e^{im\phi},  
  %\qqquad l=0,1,2,\ldots,\quad m=-l,-l+1,\ldots, l.
\end{equation*}
where \m{l=0,1,2,\ldots};~~\m{m=-l,-l+1,\ldots} and \m{P_l^m} are the associated Legendre polynomials.  
Recall that the spherical harmonics are the eignefunctions of the Laplace operator on \m{S_2} (with eigenvalue \m{-l^2}), 
and they form an orthonormal basis for \m{L_2(S_2)}, 
hence %any \m{f\in L_2(S_2)} may be represented in the form 
\begin{equation}\label{eq: Ylm exp}
  f(\theta,\phi)=\sum_{l=0}^{\infty} \sum_{m=-l}^{l} \flm{l}{m} Y_l^m(\theta,\phi)
  \qquad\text{with}\qquad 
  \flm{l}{m}=\inp{f,Y_l^m}, 
\end{equation}
where %\m{\inp{\cdot,\cdot}} denotes the inner product of functions 
\begin{equation*}
  \inp{f,g}=\int_{0}^{\pi} \int_0^{2\pi} {f^\ast\nts(\theta,\phi)}\, g(\theta,\phi) \cos\theta \:d\phi\: d\theta,  
\end{equation*}
and \m{\wbar{f}} denotes complex conjugation. 
The \m{\cbrN{\flm{l}{m}}} are called the \df{Fourier coefficients} of \m{f}, and  
in numerical computations we usually truncate them %\rf{eq: Ylm exp} 
at a finite \m{l\<= L}. 
Functions for which \m{\flm{l}{m}\<=0} for \m{l\< >L} are called \df{band-limited}. % functions on the sphere. 
%Our invariant kernel will be a function of polynomials in the \m{F_{l,m}} coefficients, which are 
%invariant under the action of \m{\SO(3)}. 
}

For a \m{\sqb{0,1}}-valued bitmap matrix M, the mapping \rf{eq: mapping} leads to  
%will have   
%via \rf{eq: mapping}, 
%the corresponding \m{\flm{l}{m}} coefficients may be computed explicitly as   %may be computed directly as a sum 
\begin{equation}\label{eq: mapping exp}
  \flm{l}{m}=c(l) \sum_{i,j=1}^{n} M_{i,j} \Ylm(\theta,\phi), 
\end{equation}
where \m{\theta=a \sqrt{x^2+y^2}}, 
\begin{equation*}
  \phi=
  \begin{cases}
    ~\arctan(y/x) & \text{if~~} y\<>0\\ 
    ~2\pi-\arctan(y/x) & \text{if~~} y\<<0\\ 
  \end{cases},
\end{equation*}
and \m{\br{x,y}=\brbig{\,\fr{i-1/2}{N}-0.5,~ \fr{j-1/2}{N}-0.5}}. 

In \rf{eq: mapping exp} we added \m{c(l)} as a smoothing device when going from the discrete bitmap to the 
(truncated) continuous representation. 
Setting \m{c(l)\equiv 1} corresponds to no smoothing, effectively representing each pixel as a delta function. 
However, because of the truncation in \m{l}, even this extreme case does not break our algorithm. 
Setting \m{c(l)=\exp(-l^2\sigma^2 /2)} corresponds to smoothing by a heat kernel on the sphere, which, 
for small enough \m{a}, closely approximates Gaussian smoothing in the orignal image plane. 
Some amount of smoothing is typically desirable, not only because because we are effectively 
performing interpolation from a discrete signal to a continuous one, but also because we are aiming for 
rotational invariance and want to avoid the appearance of artifacts due to the orientation of the original pixel grid. 
Overall, smoothing is a relatively minor technical issue in our algorithm. 

Just as the isometry group of \m{\RR^2} is \m{\ISOtwo}, the isometry group of \m{S_2} is \m{\SO(3)}, 
the group of rotations of \m{\RR^3} about the origin. It is easy to visualize that given the mapping \rf{eq: mapping},
locally, around the north pole, 
there is a one-to one corresponence between the action of \m{\SO(3)} on functions on the sphere and of 
\m{\ISOtwo} on the corresponding functions on the plane. 
In other words, any rigid motion of an image in the plane can be imitated by a 3D rotation of the corresponding 
function on \m{S_2}.   
Exploiting this, we proceed by constructing a kernel \m{\tilde k} between functions on \m{S_2} invariant to 
\m{\SO(3)} (which is a compact group) and then setting \m{k(f_1,f_2)=\tilde k(\tilde f_1,\tilde f_2)}.  
%construct our translation and rotation invariant kernel \m{k(f_1,f_2)} by 
%To simplify notation, in the following, wherever this does not become a source of ambiguity, we omit the \m{\tilde{~}} 
%symbols. 


%from above both the functions and the kernel. 


